Haves and Have-Nots: A Theory of Economic Sufficientarianism

We introduce a generalization of the concept of sufficientarianism, intended to rank allocations involving multiple consumption goods. In ranking allocations of goods for a fixed society of agents, sufficientarianism posits that allocations are compared according to the number of individuals whose consumption is deemed sufficient. We base our analysis on a novel ethical concept, which we term sufficientarian judgment. Sufficientarian judgment asserts that if in starting from an allocation in which all agents have identical consumption, a change in one agent's consumption hurts society, then there is no change in any other agent's consumption which could subsequently benefit society. Sufficientarianism is shown to be equivalent to sufficientarian judgment, symmetry, and separability. We investigate our axioms in an abstract environment, and in specific economic environments. Finally, we argue formally that sufficientarian judgment is closely related to the leximin principle.

==> latticeZ2.tex <==
\begin{tikzpicture}
\definecolor{darkgray176}{RGB}{176,176,176}
\begin{axis}[
tick align=outside,
tick pos=left,
title={Lattice on \(\displaystyle \mathbb{Z}^2\)},
x grid style={darkgray176},
xmin=-2.25, xmax=3.25,
xtick style={color=black},
y grid style={darkgray176},
ymin=-2.25, ymax=3.25,
ytick style={color=black}
]
\addplot [draw=black, fill=black, mark=*, only marks, opacity=0.5]
table{%
x  y
3 -1
3 -2
3 1
0 2
2 2
1 0
1 3
-1 -1
-2 -1
-2 -2
-1 -2
-1 1
-2 1
3 0
3 3
0 -2
0 -1
0 1
2 -1
2 -2
1 2
2 1
-2 0
-1 0
-1 3
-2 3
3 2
-1 2
0 0
1 1
0 3
2 0
1 -2
1 -1
2 3
-2 2
};
\end{axis}

\end{tikzpicture}

==> society_example.tex <==
\begin{tikzpicture}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1,0.5)},
  anchor=west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Agents},
xmajorgrids,
xmin=-0.25, xmax=5.25,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={A,B,C,D,E,F},
y grid style={darkgray176},
ylabel={Wealth Level},
ymajorgrids,
ymin=15.85, ymax=41.15,
ytick style={color=black}
]
\addplot [draw=gray, fill=gray, mark=*, only marks]
table{%
x  y
0 40
1 32
2 27
3 23
4 23
5 17
};
\addlegendentry{Society 1}
\addplot [draw=black, fill=black, mark=diamond*, only marks]
table{%
x  y
0 38
1 36
2 33
3 27
4 20
5 20
};
\addlegendentry{Society 2}
\addplot [semithick, gray]
table {%
0 30
1 30
2 30
3 30
4 30
5 30
};
\addlegendentry{$\beta$}
\end{axis}

\end{tikzpicture}

==> society_result.tex <==
\begin{tikzpicture}
\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1,0.5)},
  anchor=west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Agents},
xmajorgrids,
xmin=-0.25, xmax=5.25,
xtick style={color=black},
xtick={0,1,2,3,4,5},
xticklabels={A,B,C,D,E,F},
y grid style={darkgray176},
ylabel={Wealth Level},
ymajorgrids,
ymin=15.85, ymax=41.15,
ytick style={color=black}
]

\addplot [draw=gray, fill=gray, mark=*, only marks]
table{%
x  y
0 40
1 32
2 27
3 23
4 23
5 17
};
\addlegendentry{Society 1}
\addplot [draw=black, fill=black, mark=diamond*, only marks]
table{%
x  y
0 38
1 36
2 33
3 27
4 20
5 20
};
\addlegendentry{Society 2}
\addplot [semithick, gray]
table {%
0 30
1 30
2 30
3 30
4 30
5 30
};
\addlegendentry{$\beta$}
\addplot [semithick, steelblue31119180, mark=o, mark size=7.5, mark options={solid,fill opacity=0,draw=black}, only marks, forget plot]
table {%
0 38
};
\addplot [semithick, darkorange25512714, mark=o, mark size=7.5, mark options={solid,fill opacity=0,draw=black}, only marks, forget plot]
table {%
1 32
};
\addplot [semithick, forestgreen4416044, mark=o, mark size=7.5, mark options={solid,fill opacity=0,draw=black}, only marks, forget plot]
table {%
2 27
};
\addplot [semithick, crimson2143940, mark=o, mark size=7.5, mark options={solid,fill opacity=0,draw=black}, only marks, forget plot]
table {%
3 23
};
\addplot [semithick, mediumpurple148103189, mark=o, mark size=7.5, mark options={solid,fill opacity=0,draw=black}, only marks, forget plot]
table {%
4 20
};
\addplot [semithick, sienna1408675, mark=o, mark size=7.5, mark options={solid,fill opacity=0,draw=black}, only marks, forget plot]
table {%
5 17
};
\end{axis}

\end{tikzpicture}
